Learning to Disentangle Robust and Vulnerable Features for Adversarial Detection

Although deep neural networks have shown promising performances on various tasks, even achieving human-level performance on some, they are shown to be susceptible to incorrect predictions even with imperceptibly small perturbations to an input. There exists a large number of previous works which proposed to defend against such adversarial attacks either by robust inference or detection of adversarial inputs. Yet, most of them cannot effectively defend against whitebox attacks where an adversary has a knowledge of the model and defense. More importantly, they do not provide a convincing reason why the generated adversarial inputs successfully fool the target models. To address these shortcomings of the existing approaches, we hypothesize that the adversarial inputs are tied to latent features that are susceptible to adversarial perturbation, which we call vulnerable features. Then based on this intuition, we propose a minimax game formulation to disentangle the latent features of each instance into robust and vulnerable ones, using variational autoencoders with two latent spaces. We thoroughly validate our model for both blackbox and whitebox attacks on MNIST, Fashion MNIST5, and Cat & Dog datasets, whose results show that the adversarial inputs cannot bypass our detector without changing its semantics, in which case the attack has failed.

==> Makefile <==
MAIN ?= p
DIFF ?= HEAD^
CODE := $(addsuffix .tex,$(filter-out %.tex,$(wildcard code/*)))
FIGS := $(patsubst %.svg,%.pdf,$(wildcard svgfig/*.svg))
PPTX := $(patsubst pptx/%.pdf,fig/%-crop.pdf,$(wildcard pptx/*.pdf))
PLOT := $(patsubst %.gp,%.tex,$(wildcard data/*.gp))
DEPS := rev.tex code/fmt.tex abstract.txt $(CODE) $(FIGS) $(PPTX) $(PLOT)
BTEX := --bibtex-args="-min-crossrefs=99"
LTEX := --latex-args="-interaction=nonstopmode -synctex=4"
SHELL:= $(shell echo $$SHELL)

all: $(DEPS) ## generate a pdf
	@TEXINPUTS="sty:" python3 bin/latexrun.py $(BTEX) $(LTEX) $(MAIN)
	@ln -sf latex.out/p.synctex.gz p.synctex.gz

submit: $(DEPS) ## proposal function
	@for f in $(wildcard submit-*.tex); do \
		TEXINPUTS="sty:" python3 bin/latexrun.py $$f; \
	done

diff: $(DEPS) ## generate diff-highlighed pdf
	@bin/diff.sh $(DIFF)

help: ## print help
	@grep -E '^[a-zA-Z_-]+:.*?## .*$$' $(MAKEFILE_LIST) \
	  | sort | awk 'BEGIN {FS = ":.*?## "}; {printf "\033[36m%-10s\033[0m %s\n", $$1, $$2}'

rev.tex: FORCE
	@printf '\\gdef\\therev{%s}\n\\gdef\\thedate{%s}\n' \
	   "$(shell git rev-parse --short HEAD)"            \
	   "$(shell git log -1 --format='%ci' HEAD)" > $@

code/%.tex: code/% ## build highlighted tex code from source code
	pygmentize -P tabsize=4 -P mathescape -f latex $^ > $@

code/fmt.tex: ## generate color table
	pygmentize -f latex -S default > $@

svgfig/%.pdf: svgfig/%.svg ## generate pdf from svg
	inkscape --without-gui -f $^ -D -A $@

fig/%-crop.pdf: pptx/%.pdf
	pdfcrop --margin=1 $^ $@

graphs:
	echo "Building Graphs"
	(cd graphs && ./run.sh)

data/%.tex: data/%.gp ## generate plot
	gnuplot $^

draft: $(DEPS) ## generate pdf with a draft info
	echo -e '\\newcommand*{\\DRAFT}{}' >> rev.tex
	@TEXINPUTS="sty:" python3 bin/latexrun.py $(BTEX) $(MAIN)

watermark: $(DEPS) ## generate pdf with a watermark
	echo -e '\\usepackage[firstpage]{draftwatermark}' >> rev.tex
	@TEXINPUTS="sty:" python3 bin/latexrun.py $(BTEX) $(MAIN)

spell: ## run a spell check
	@for i in *.tex; do bin/aspell.sh $$i; done
	@for i in *.tex; do bin/double.pl $$i; done
	@for i in *.tex; do bin/abbrv.pl  $$i; done
	@bin/hyphens.sh *.tex
	@pdftotext $(MAIN).pdf /dev/stdout | grep '??'

clean: ## clean up
	@python3 bin/latexrun.py --clean
	rm -f abstract.txt

distclean: clean ## clean up completely
	rm -f code/*.tex

init: ## init writing (discarding example)
	rm -f {code,fig,data}/ex-*
	perl -pi -e 's/^\\input{ex}/% \\input{ex}/g' $(MAIN).tex

abstract.txt: abstract.tex $(MAIN).tex ## generate abstract.txt
	@python3 bin/mkabstract.py $(MAIN).tex $< | fmt -w72 > $@

.PHONY: all help FORCE draft clean spell distclean init


==> code/Makefile.tex <==
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`\$=3\catcode`\^=7\catcode`\_=8}]
\PY{n+nf}{all}\PY{o}{:}
    \PY{o}{(}\PY{n+nb}{cd} .. \PY{o}{\PYZam{}\PYZam{}} make\PY{o}{)}
\end{Verbatim}


==> code/attr.c.tex <==
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`\$=3\catcode`\^=7\catcode`\_=8}]
\PY{k+kt}{int} \PY{n}{sensitive\PYZus{}data}\PY{p}{[}\PY{l+m+mi}{1024}\PY{p}{]} \PY{n}{\PYZus{}\PYZus{}attribute\PYZus{}\PYZus{}}\PY{p}{(}\PY{p}{(}\PY{n}{oblivious}\PY{p}{)}\PY{p}{)}\PY{p}{;}

\PY{c+c1}{// attribute setting to indicate sensitive function}
\PY{k+kt}{void} \PY{n+nf}{sensitive\PYZus{}function}\PY{p}{(}\PY{k+kt}{int} \PY{n}{arg1}\PY{p}{)} \PY{n}{\PYZus{}\PYZus{}attribute\PYZus{}\PYZus{}}\PY{p}{(}\PY{p}{(}\PY{n}{oblivious}\PY{p}{)}\PY{p}{)} \PY{p}{\PYZob{}}
\PY{p}{.}\PY{p}{.}\PY{p}{.}
\PY{p}{\PYZcb{}}
\end{Verbatim}


==> code/avx-reg.asm.tex <==
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`\$=3\catcode`\^=7\catcode`\_=8}]
\PY{c+c1}{; \PYZpc{}rsi points to the base address of ORAM tree block.}
\PY{n+nf}{movaps} \PY{p}{(}\PY{o}{\PYZpc{}}\PY{n+nb}{rsi}\PY{p}{),} \PY{o}{\PYZpc{}}\PY{n+nv}{xmm0}
\PY{n+nf}{vinserti128} \PY{k+kc}{\PYZdl{}}\PY{l+m+mh}{0x0}\PY{p}{,} \PY{o}{\PYZpc{}}\PY{n+nv}{xmm0}\PY{p}{,} \PY{o}{\PYZpc{}}\PY{n+nv}{ymm5}\PY{p}{,} \PY{o}{\PYZpc{}}\PY{n+nv}{ymm5}
\PY{n+nf}{add} \PY{k+kc}{\PYZdl{}}\PY{l+m+mi}{16}\PY{p}{,} \PY{o}{\PYZpc{}}\PY{n+nb}{rsi}
\PY{n+nf}{movaps} \PY{p}{(}\PY{o}{\PYZpc{}}\PY{n+nb}{rsi}\PY{p}{),} \PY{o}{\PYZpc{}}\PY{n+nv}{xmm0}
\PY{n+nf}{vinserti128} \PY{k+kc}{\PYZdl{}}\PY{l+m+mh}{0x1}\PY{p}{,} \PY{o}{\PYZpc{}}\PY{n+nv}{xmm0}\PY{p}{,} \PY{o}{\PYZpc{}}\PY{n+nv}{ymm5}\PY{p}{,} \PY{o}{\PYZpc{}}\PY{n+nv}{ymm5}
\PY{n+nf}{add} \PY{k+kc}{\PYZdl{}}\PY{l+m+mi}{16}\PY{p}{,} \PY{o}{\PYZpc{}}\PY{n+nb}{rsi}
\PY{n+nf}{movaps} \PY{p}{(}\PY{o}{\PYZpc{}}\PY{n+nb}{rsi}\PY{p}{),} \PY{o}{\PYZpc{}}\PY{n+nv}{xmm0}
\PY{n+nf}{vinserti128} \PY{k+kc}{\PYZdl{}}\PY{l+m+mh}{0x0}\PY{p}{,} \PY{o}{\PYZpc{}}\PY{n+nv}{xmm0}\PY{p}{,} \PY{o}{\PYZpc{}}\PY{n+nv}{ymm6}\PY{p}{,} \PY{o}{\PYZpc{}}\PY{n+nv}{ymm6}
\PY{n+nf}{add} \PY{k+kc}{\PYZdl{}}\PY{l+m+mi}{16}\PY{p}{,} \PY{o}{\PYZpc{}}\PY{n+nb}{rsi}
\PY{n+nf}{movaps} \PY{p}{(}\PY{o}{\PYZpc{}}\PY{n+nb}{rsi}\PY{p}{),} \PY{o}{\PYZpc{}}\PY{n+nv}{xmm0}
\PY{n+nf}{vinserti128} \PY{k+kc}{\PYZdl{}}\PY{l+m+mh}{0x1}\PY{p}{,} \PY{o}{\PYZpc{}}\PY{n+nv}{xmm0}\PY{p}{,} \PY{o}{\PYZpc{}}\PY{n+nv}{ymm6}\PY{p}{,} \PY{o}{\PYZpc{}}\PY{n+nv}{ymm6}
\end{Verbatim}


==> code/bp.c.tex <==
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`\$=3\catcode`\^=7\catcode`\_=8}]
\PY{k+kt}{void} \PY{n+nf}{func\PYZus{}one}\PY{p}{(}\PY{p}{)} \PY{p}{\PYZob{}}
  \PY{k}{return}\PY{p}{;}
\PY{p}{\PYZcb{}}

\PY{k+kt}{void} \PY{n+nf}{func\PYZus{}two}\PY{p}{(}\PY{p}{)} \PY{p}{\PYZob{}}
  \PY{k}{return}\PY{p}{;}
\PY{p}{\PYZcb{}}

\PY{k+kt}{void} \PY{n+nf}{start\PYZus{}func}\PY{p}{(}\PY{p}{)} \PY{p}{\PYZob{}}
  \PY{k+kt}{int} \PY{n}{opt} \PY{o}{=} \PY{l+m+mi}{0}\PY{p}{;}
  \PY{k}{for} \PY{p}{(}\PY{k+kt}{int} \PY{n}{i} \PY{o}{=} \PY{l+m+mi}{0}\PY{p}{;} \PY{n}{i} \PY{o}{\PYZlt{}} \PY{l+m+mi}{50}\PY{p}{;} \PY{n}{i}\PY{o}{+}\PY{o}{+}\PY{p}{)} \PY{p}{\PYZob{}}
    \PY{k}{if} \PY{p}{(}\PY{n}{i}\PY{o}{\PYZpc{}}\PY{l+m+mi}{2} \PY{o}{=}\PY{o}{=} \PY{l+m+mi}{0}\PY{p}{)}
      \PY{n}{func\PYZus{}one}\PY{p}{;}
    \PY{k}{else}
      \PY{n}{func\PYZus{}two}\PY{p}{;}
  \PY{p}{\PYZcb{}}
\PY{p}{\PYZcb{}}
\end{Verbatim}


==> code/fmt.tex <==
\makeatletter
\def\PY@reset{\let\PY@it=\relax \let\PY@bf=\relax%
    \let\PY@ul=\relax \let\PY@tc=\relax%
    \let\PY@bc=\relax \let\PY@ff=\relax}
\def\PY@tok#1{\csname PY@tok@#1\endcsname}
\def\PY@toks#1+{\ifx\relax#1\empty\else%
    \PY@tok{#1}\expandafter\PY@toks\fi}
\def\PY@do#1{\PY@bc{\PY@tc{\PY@ul{%
    \PY@it{\PY@bf{\PY@ff{#1}}}}}}}
\def\PY#1#2{\PY@reset\PY@toks#1+\relax+\PY@do{#2}}

\expandafter\def\csname PY@tok@gd\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.63,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@gu\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.50,0.00,0.50}{##1}}}
\expandafter\def\csname PY@tok@gt\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.27,0.87}{##1}}}
\expandafter\def\csname PY@tok@gs\endcsname{\let\PY@bf=\textbf}
\expandafter\def\csname PY@tok@gr\endcsname{\def\PY@tc##1{\textcolor[rgb]{1.00,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@cm\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@vg\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@vi\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@vm\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@mh\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@cs\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@ge\endcsname{\let\PY@it=\textit}
\expandafter\def\csname PY@tok@vc\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@il\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@go\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.53,0.53,0.53}{##1}}}
\expandafter\def\csname PY@tok@cp\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.74,0.48,0.00}{##1}}}
\expandafter\def\csname PY@tok@gi\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.63,0.00}{##1}}}
\expandafter\def\csname PY@tok@gh\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,0.50}{##1}}}
\expandafter\def\csname PY@tok@ni\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.60,0.60,0.60}{##1}}}
\expandafter\def\csname PY@tok@nl\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.63,0.63,0.00}{##1}}}
\expandafter\def\csname PY@tok@nn\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@no\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.53,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@na\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.49,0.56,0.16}{##1}}}
\expandafter\def\csname PY@tok@nb\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@nc\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@nd\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.67,0.13,1.00}{##1}}}
\expandafter\def\csname PY@tok@ne\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.82,0.25,0.23}{##1}}}
\expandafter\def\csname PY@tok@nf\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@si\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.73,0.40,0.53}{##1}}}
\expandafter\def\csname PY@tok@s2\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@nt\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@nv\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@s1\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@dl\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@ch\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@m\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@gp\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,0.50}{##1}}}
\expandafter\def\csname PY@tok@sh\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@ow\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.67,0.13,1.00}{##1}}}
\expandafter\def\csname PY@tok@sx\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@bp\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@c1\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@fm\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@o\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@kc\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@c\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@mf\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@err\endcsname{\def\PY@bc##1{\setlength{\fboxsep}{0pt}\fcolorbox[rgb]{1.00,0.00,0.00}{1,1,1}{\strut ##1}}}
\expandafter\def\csname PY@tok@mb\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@ss\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@sr\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.40,0.53}{##1}}}
\expandafter\def\csname PY@tok@mo\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@kd\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@mi\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@kn\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@cpf\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@kr\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@s\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@kp\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@w\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.73,0.73}{##1}}}
\expandafter\def\csname PY@tok@kt\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.69,0.00,0.25}{##1}}}
\expandafter\def\csname PY@tok@sc\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@sb\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@sa\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@k\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@se\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.73,0.40,0.13}{##1}}}
\expandafter\def\csname PY@tok@sd\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}

\def\PYZbs{\char`\\}
\def\PYZus{\char`\_}
\def\PYZob{\char`\{}
\def\PYZcb{\char`\}}
\def\PYZca{\char`\^}
\def\PYZam{\char`\&}
\def\PYZlt{\char`\<}
\def\PYZgt{\char`\>}
\def\PYZsh{\char`\#}
\def\PYZpc{\char`\%}
\def\PYZdl{\char`\$}
\def\PYZhy{\char`\-}
\def\PYZsq{\char`\'}
\def\PYZdq{\char`\"}
\def\PYZti{\char`\~}
% for compatibility with earlier versions
\def\PYZat{@}
\def\PYZlb{[}
\def\PYZrb{]}
\makeatother



==> code/inst-call.asm.tex <==
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`\$=3\catcode`\^=7\catcode`\_=8}]
\PY{c+c1}{; Before}
  \PY{n+nf}{call} \PY{n+nv}{function\PYZus{}addr}  

\PY{c+c1}{; After}
  \PY{n+nf}{sub} \PY{n+nv}{R13}\PY{p}{,} \PY{l+m+mi}{8}                \PY{c+c1}{; Adjust ORAM stack address}
  \PY{n+nf}{mov} \PY{n+nv}{R15}\PY{p}{,} \PY{n+nv}{R13}              \PY{c+c1}{; Pass the ORAM stack top address}
  \PY{n+nf}{mov} \PY{n+nv}{R14}\PY{p}{,} \PY{n+nv}{after\PYZus{}fetch}      \PY{c+c1}{; Psss the return address after fetch}
  \PY{n+nf}{jmp} \PY{n+nv}{data\PYZus{}oram\PYZus{}controller}  \PY{c+c1}{; Fetch the stack basic block to D\PYZhy{}pad}
\PY{n+nl}{after\PYZus{}fetch:}
  \PY{n+nf}{mov} \PY{p}{(}\PY{n+nv}{R15}\PY{p}{),} \PY{n+nv}{return\PYZus{}addr}    \PY{c+c1}{; Now R15 is a stack top address on D\PYZhy{}pad}
                            \PY{c+c1}{; save the return\PYZus{}addr}

  \PY{n+nf}{mov} \PY{n+nv}{R15}\PY{p}{,} \PY{n+nv}{function\PYZus{}addr}    \PY{c+c1}{; Pass call address}
  \PY{n+nf}{jmp} \PY{n+nv}{code\PYZus{}oram\PYZus{}controller}  \PY{c+c1}{; Fetch the code basic block to C\PYZhy{}pad}
                            \PY{c+c1}{; then, jump to the start of C\PYZhy{}pad}
\PY{n+nl}{return\PYZus{}addr:}
\end{Verbatim}


==> code/inst-cond.asm.tex <==
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`\$=3\catcode`\^=7\catcode`\_=8}]
\PY{c+c1}{; Before}
  \PY{n+nf}{jne} \PY{n+nv}{L1}
\PY{n+nl}{L2:}

\PY{c+c1}{; After}
  \PY{n+nf}{mov} \PY{n+nv}{R14}\PY{p}{,} \PY{n+nv}{L1}              \PY{c+c1}{; L1 : jump target }
  \PY{n+nf}{mov} \PY{n+nv}{R15}\PY{p}{,} \PY{n+nv}{L2}              \PY{c+c1}{; L2 : fallthrough}
  \PY{n+nf}{cmovne} \PY{n+nv}{R15}\PY{p}{,} \PY{n+nv}{r14}          \PY{c+c1}{; R15 holds an evaluated target (L1 or L2)}
  \PY{n+nf}{jmp} \PY{n+nv}{code\PYZus{}oram\PYZus{}controller} \PY{c+c1}{; Fetch the code basic block to C\PYZhy{}pad}
                           \PY{c+c1}{; then, jump to the start of C\PYZhy{}pad}
\PY{n+nl}{L2:}
\end{Verbatim}


==> code/inst-pop.asm.tex <==
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`\$=3\catcode`\^=7\catcode`\_=8}]
\PY{c+c1}{; Before}
  \PY{n+nf}{pop64r} \PY{n+nv}{reg} 

\PY{c+c1}{; After}
  \PY{n+nf}{mov} \PY{n+nv}{R15}\PY{p}{,} \PY{n+nv}{R13}                \PY{c+c1}{; Pass ORAM stack pointer to R15}
  \PY{n+nf}{mov} \PY{n+nv}{R14}\PY{p}{,} \PY{n+nv}{after\PYZus{}fetch}        \PY{c+c1}{; Pass the return address}
  \PY{n+nf}{jmp} \PY{n+nv}{data\PYZus{}oram\PYZus{}controller}    \PY{c+c1}{; Data ORAM controller updates D\PYZhy{}pad }
\PY{n+nl}{after\PYZus{}fetch:}
  \PY{n+nf}{mov} \PY{n+nv}{reg}\PY{p}{,} \PY{p}{(}\PY{n+nv}{R15}\PY{p}{)}              \PY{c+c1}{; Read value from D\PYZhy{}pad}
  \PY{n+nf}{add} \PY{n+nv}{R13}\PY{p}{,} \PY{l+m+mi}{8}                  \PY{c+c1}{; Adjust the stack pointer}
\end{Verbatim}


==> code/inst-push.asm.tex <==
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`\$=3\catcode`\^=7\catcode`\_=8}]
\PY{c+c1}{; Before}
  \PY{n+nf}{push64r} \PY{n+nv}{reg}

\PY{c+c1}{; After}
  \PY{n+nf}{sub} \PY{n+nv}{R13}\PY{p}{,} \PY{l+m+mi}{8}                  \PY{c+c1}{; Reserve ORAM stack}
  \PY{n+nf}{mov} \PY{n+nv}{R15}\PY{p}{,} \PY{n+nv}{R13}                \PY{c+c1}{; Pass stack pointer via R15}
  \PY{n+nf}{mov} \PY{n+nv}{R14}\PY{p}{,} \PY{n+nv}{after\PYZus{}fecth}        \PY{c+c1}{; Pass the return address}
  \PY{n+nf}{jmp} \PY{n+nv}{data\PYZus{}oram\PYZus{}controller}    \PY{c+c1}{; Data ORAM controller updates D\PYZhy{}pad }
\PY{n+nl}{after\PYZus{}fetch:}
  \PY{n+nf}{mov} \PY{p}{(}\PY{n+nv}{R15}\PY{p}{),} \PY{n+nv}{reg}              \PY{c+c1}{; R15 is now D\PYZhy{}pad address and}
                              \PY{c+c1}{; Write reg to stack top on the D\PYZhy{}pad}
\end{Verbatim}


==> code/inst-return.asm.tex <==
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`\$=3\catcode`\^=7\catcode`\_=8}]
\PY{c+c1}{; Before}
  \PY{n+nf}{return}

\PY{c+c1}{; After}
  \PY{n+nf}{mov} \PY{n+nv}{R15}\PY{p}{,} \PY{n+nv}{R13}                \PY{c+c1}{; Pass the ORAM stack top address }
  \PY{n+nf}{mov} \PY{n+nv}{R14}\PY{p}{,} \PY{n+nv}{return\PYZus{}addr}        \PY{c+c1}{; Pass the return address after fetch}
  \PY{n+nf}{jmp} \PY{n+nv}{data\PYZus{}oram\PYZus{}controller}    \PY{c+c1}{; Fetch the stack basic block to D\PYZhy{}pad}
\PY{n+nl}{after\PYZus{}fetch:}
  \PY{n+nf}{mov} \PY{n+nv}{R14}\PY{p}{,} \PY{n+nv}{R15}                \PY{c+c1}{; Move the D\PYZhy{}pad address to R14}
  \PY{n+nf}{mov} \PY{n+nv}{R15}\PY{p}{,} \PY{p}{(}\PY{n+nv}{R14}\PY{p}{)}              \PY{c+c1}{; Read the return address from D\PYZhy{}pad }
  \PY{n+nf}{add} \PY{n+nv}{R13}\PY{p}{,} \PY{l+m+mi}{8}                  \PY{c+c1}{; Adjust the stack pointer}
  \PY{n+nf}{jmp} \PY{n+nv}{code\PYZus{}oram\PYZus{}controller}    \PY{c+c1}{; Fetch the code basic block to C\PYZhy{}pad }
                              \PY{c+c1}{; then, jump to the start of C\PYZhy{}pad}
\end{Verbatim}


==> code/inst-store.asm.tex <==
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`\$=3\catcode`\^=7\catcode`\_=8}]
\PY{c+c1}{; Before}
  \PY{n+nf}{mov} \PY{l+m+mi}{4}\PY{p}{(}\PY{n+nb}{RAX}\PY{p}{),} \PY{n+nb}{RBX}           \PY{c+c1}{; Store RBX at where (RAX + 4) points to}

\PY{c+c1}{; After}
  \PY{n+nf}{lea} \PY{n+nv}{R15}\PY{p}{,} \PY{l+m+mi}{4}\PY{p}{(}\PY{n+nb}{RAX}\PY{p}{)}           \PY{c+c1}{; Pass the store address through R15}
  \PY{n+nf}{mov} \PY{n+nv}{R14}\PY{p}{,} \PY{n+nv}{after\PYZus{}fetch}      \PY{c+c1}{; Pass the return address through R14}
  \PY{n+nf}{jmp} \PY{n+nv}{data\PYZus{}oram\PYZus{}controller}  \PY{c+c1}{; data\PYZus{}oram\PYZus{}controller fetches data block}
                            \PY{c+c1}{; and returns address of (D\PYZhy{}Pad + offset)}
                            \PY{c+c1}{; through R15}
\PY{n+nl}{after\PYZus{}fetch:}
  \PY{n+nf}{mov} \PY{p}{(}\PY{n+nv}{R15}\PY{p}{),} \PY{n+nb}{RBX}            \PY{c+c1}{; Write a value RBX to (D\PYZhy{}Pad + offset)}
\end{Verbatim}


==> code/inst-uncond.asm.tex <==
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`\$=3\catcode`\^=7\catcode`\_=8}]
\PY{c+c1}{; Before}
  \PY{n+nf}{jmp} \PY{n+nv}{jump\PYZus{}target}

\PY{c+c1}{; After}
  \PY{n+nf}{mov} \PY{n+nv}{R15}\PY{p}{,} \PY{n+nv}{jump\PYZus{}target}        \PY{c+c1}{; Pass jump\PYZus{}target through R15}
  \PY{n+nf}{jmp} \PY{n+nv}{code\PYZus{}oram\PYZus{}controller}    \PY{c+c1}{; code\PYZus{}oram\PYZus{}controller loads the code}
                              \PY{c+c1}{; block to C\PYZhy{}Pad and then jumps to the}
                              \PY{c+c1}{; beginning of C\PYZhy{}Pad.}
\end{Verbatim}


==> code/oram-secure.c.tex <==
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`\$=3\catcode`\^=7\catcode`\_=8}]
\PY{k+kt}{void} \PY{n+nf}{retrieve\PYZus{}from\PYZus{}stash\PYZus{}cmov}\PY{p}{(}\PY{k+kt}{void}\PY{o}{*} \PY{n}{cpad}\PY{p}{,} \PY{k+kt}{int} \PY{n}{required\PYZus{}blk}\PY{p}{)} \PY{p}{\PYZob{}}
  \PY{k+kt}{bool} \PY{n}{flag} \PY{o}{=} \PY{n+nb}{false}\PY{p}{;}

  \PY{k}{for} \PY{p}{(}\PY{k+kt}{int} \PY{n}{i} \PY{o}{=} \PY{l+m+mi}{0}\PY{p}{;} \PY{n}{i} \PY{o}{\PYZlt{}} \PY{n}{NUM\PYZus{}STASH\PYZus{}BLOCKS}\PY{p}{;} \PY{n}{i}\PY{o}{+}\PY{o}{+}\PY{p}{)} \PY{p}{\PYZob{}}
    \PY{c+c1}{// Check the validity of the condition, i.e.,}
    \PY{c+c1}{// is this the block to retrieve from the stash}
    \PY{n}{flag} \PY{o}{=} \PY{p}{(}\PY{p}{(}\PY{n}{stash}\PY{p}{[}\PY{n}{i}\PY{p}{]}\PY{p}{.}\PY{n}{blocknum} \PY{o}{=}\PY{o}{=} \PY{n}{required\PYZus{}blk}\PY{p}{)}\PY{p}{)}\PY{p}{;}

    \PY{c+c1}{// Based on the flag, either perform a real or a dummy copy}
    \PY{n}{x86\PYZus{}cmov}\PY{p}{(}\PY{n}{cpad}\PY{p}{,} \PY{n}{stash}\PY{p}{[}\PY{n}{i}\PY{p}{]}\PY{p}{.}\PY{n}{memblk}\PY{p}{,} \PY{n}{flag}\PY{p}{)}\PY{p}{;}
  \PY{p}{\PYZcb{}}
\PY{p}{\PYZcb{}}
\end{Verbatim}


==> code/shuffle.py.tex <==
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`\$=3\catcode`\^=7\catcode`\_=8}]
\PY{k}{def} \PY{n+nf}{shuffle}\PY{p}{(}\PY{n}{addr1}\PY{p}{,} \PY{n}{addr2}\PY{p}{,} \PY{n}{size}\PY{p}{)}\PY{p}{:}
  \PY{c+c1}{\PYZsh{} Find and update table entries}
  \PY{n}{entry1} \PY{o}{=} \PY{n}{find\PYZus{}entry}\PY{p}{(}\PY{n}{addr1}\PY{p}{)}
  \PY{n}{entry1}\PY{o}{.}\PY{n}{addr} \PY{o}{=} \PY{n}{addr2}
  \PY{n}{entry1}\PY{o}{.}\PY{n}{size} \PY{o}{=} \PY{n}{size}

  \PY{n}{entry2} \PY{o}{=} \PY{n}{find\PYZus{}entry}\PY{p}{(}\PY{n}{addr2}\PY{p}{)}
  \PY{n}{entry2}\PY{o}{.}\PY{n}{addr} \PY{o}{=} \PY{n}{addr1}
  \PY{n}{entry2}\PY{o}{.}\PY{n}{size} \PY{o}{=} \PY{n}{size}

  \PY{c+c1}{\PYZsh{} Lock table entries}
  \PY{n}{lock}\PY{p}{(}\PY{n}{entry1}\PY{o}{.}\PY{n}{lock}\PY{p}{)}
  \PY{n}{lock}\PY{p}{(}\PY{n}{entry2}\PY{o}{.}\PY{n}{lock}\PY{p}{)}

  \PY{n}{ShuffleQueue}\PY{o}{.}\PY{n}{append}\PY{p}{(}\PY{p}{(}\PY{n}{entry1}\PY{p}{,} \PY{n}{entry2}\PY{p}{,} \PY{n}{size}\PY{p}{)}\PY{p}{)}
  \PY{k}{return}

\PY{k}{def} \PY{n+nf}{shuffle\PYZus{}background}\PY{p}{(}\PY{p}{)}\PY{p}{:}
  \PY{c+c1}{\PYZsh{} Iterate over all entries in the queue}
  \PY{k}{while} \PY{n+nb+bp}{True}\PY{p}{:}
    \PY{c+c1}{\PYZsh{} Pop a queued item}
    \PY{p}{(}\PY{n}{entry1}\PY{p}{,} \PY{n}{entry2}\PY{p}{,} \PY{n}{size}\PY{p}{)} \PY{o}{=} \PY{n}{ShuffleQueue}\PY{o}{.}\PY{n}{pop}\PY{p}{(}\PY{p}{)}

    \PY{c+c1}{\PYZsh{} Shuffles the data}
    \PY{n}{memcpy}\PY{p}{(}\PY{n}{tmp}\PY{p}{,} \PY{n}{entry1}\PY{o}{.}\PY{n}{addr}\PY{p}{,} \PY{n}{size}\PY{p}{)}
    \PY{n}{memcpy}\PY{p}{(}\PY{n}{entry1}\PY{o}{.}\PY{n}{addr}\PY{p}{,} \PY{n}{entry2}\PY{o}{.}\PY{n}{addr}\PY{p}{,} \PY{n}{size}\PY{p}{)}
    \PY{n}{memcpy}\PY{p}{(}\PY{n}{entry2}\PY{o}{.}\PY{n}{addr}\PY{p}{,} \PY{n}{tmp}\PY{p}{,} \PY{n}{size}\PY{p}{)}

    \PY{c+c1}{\PYZsh{} Unlock table entries}
    \PY{n}{unlock}\PY{p}{(}\PY{n}{entry1}\PY{o}{.}\PY{n}{lock}\PY{p}{)}
    \PY{n}{unlock}\PY{p}{(}\PY{n}{entry2}\PY{o}{.}\PY{n}{lock}\PY{p}{)}
  \PY{k}{return}
\end{Verbatim}


==> code/stack-frame.asm.tex <==
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`\$=3\catcode`\^=7\catcode`\_=8}]
\PY{c+c1}{; Before (function prologue)}
\PY{n+nf}{push} \PY{n+nb}{RBP}
\PY{n+nf}{mov} \PY{n+nb}{RBP}\PY{p}{,} \PY{n+nb}{RSP}
\PY{n+nf}{...} 
\PY{c+c1}{; Before (function epilogue)}
\PY{n+nf}{pop} \PY{n+nb}{RBP}
\PY{n+nf}{return}

\PY{c+c1}{; After (function prologue)}
\PY{n+nf}{push} \PY{n+nb}{RBP}        
\PY{n+nf}{mov} \PY{n+nb}{RBP}\PY{p}{,} \PY{n+nb}{RSP}
\PY{n+nf}{rdrand} \PY{n+nb}{R15D}
\PY{n+nf}{and} \PY{n+nb}{R15D}\PY{p}{,} \PY{l+m+mh}{0x00f0}
\PY{n+nf}{sub} \PY{n+nv}{R15}\PY{p}{,} \PY{n+nb}{RSP}
\PY{n+nf}{...}         
\PY{c+c1}{; After (function epilogue)}
\PY{n+nf}{mov} \PY{n+nb}{RBP}\PY{p}{,} \PY{n+nb}{RSP}        
\PY{n+nf}{pop} \PY{n+nb}{RBP}
\PY{n+nf}{return}        
\end{Verbatim}


==> rev.tex <==
\gdef\therev{}
\gdef\thedate{}

